Double Mixture: Towards Continual Event Detection from Speech

Speech event detection is crucial for multimedia retrieval, involving the tagging of both semantic and acoustic events. Traditional ASR systems often overlook the interplay between these events, focusing solely on content, even though the interpretation of dialogue can vary with environmental context. This paper tackles two primary challenges in speech event detection: the continual integration of new events without forgetting previous ones, and the disentanglement of semantic from acoustic events. We introduce a new task, continual event detection from speech, for which we also provide two benchmark datasets. To address the challenges of catastrophic forgetting and effective disentanglement, we propose a novel method, 'Double Mixture.' This method merges speech expertise with robust memory mechanisms to enhance adaptability and prevent forgetting. Our comprehensive experiments show that this task presents significant challenges that are not effectively addressed by current state-of-the-art methods in either computer vision or natural language processing. Our approach achieves the lowest rates of forgetting and the highest levels of generalization, proving robust across various continual learning sequences. Our code and data are available at https://anonymous.4open.science/status/Continual-SpeechED-6461.

==> figure/DM-algorithm.tex <==

\begin{algorithm}
\caption{Training phase}
\begin{algorithmic}[1]
\Statex \textbf{Require}: The task sequence $\mathcal{T}=\left \{ \mathcal{T}_1, \dots, \mathcal{T}_t, \dots, \mathcal{T}_T \right \}$ 
\Statex \textbf{Require}: Mixture of memory buffer $\mathcal{M}$, Mixture of speech experts $\mathcal{E}$
\Statex \textbf{Require}: Generation model $f_{\theta}$, Learning rate $\beta$
% \Statex \textbf{Require}: The mixture of speech experts $\mathcal{E}=\left \{ \mathcal{E}_1, \dots, \mathcal{E}_t, \dots, \mathcal{E}_T \right \}$
% \Statex \textbf{Require}: The mixture of speech experts module $g_{\phi}$
% \State \textbf{Initialize} $\theta$ and $\phi$
\State \textbf{Initialize} $\theta$
\For {current task $\mathcal{T}_t \in \mathcal{T}$}
    \State $\theta_t \gets \theta$
    % \State $\phi_t \gets \phi$
    \While{not convergence}
        \State \textbf{Set} $\mathcal{D}_t^{train} \gets \mathcal{D}_t^{train} \cup \mathcal{M}$
        \For{each class $\mathcal{C}_i$ in $\mathcal{T}_t$}
            \State \textbf{Initialize} $\theta_{t,i} \gets \theta_t$
            \State \textbf{Sample} $\mathcal{D}_{t,i}^{train}$ from $\mathcal{D}_t^{train}$ with $\mathcal{C}_i$
            \For {each expert $\mathcal{E}_j \in \mathcal{E}$}
                \State \textbf{Compute} the weight of each expert $\alpha_j$
                \State \textbf{Compute} experts' output $O$
            \EndFor
            \State \textbf{Evaluate} $\nabla_{\theta_{t,i}} \mathcal{L}_{\mathcal{C}_i}(f_{\theta_{t,i}})$ on $\mathcal{D}_{t,i}^{train}$
            \State \textbf{Update} $\theta_{t,i}'$ = $ AdamW(\theta_{t,i}, \mathcal{L}_{\mathcal{C}_i}(f_{\theta_{t,i}}), \beta)$ 
        \EndFor
    \EndWhile
\EndFor
\end{algorithmic}
\end{algorithm}

==> figure/res-bottleneck.tex <==

\begin{figure}[h]
  \centering
    % \fbox{\rule{0pt}{2.5in} \rule{0.9\linewidth}{0pt}}
    \includegraphics[width=0.5 \textwidth]{image/CH4-Res-bottleneck-en.pdf}
    \caption{Ablation on expert bottleneck.}
    \Description{ToDo}
    \label{fig:res-bottleneck}
\end{figure}

==> section/7-limits.tex <==
\section*{Limitations}
This paper may have two limitations: (1) The investigation concentrates on audio samples predominantly less than 15 seconds in duration. One significant challenge faced in the speech community is efficiently processing lengthy audio signals due to limitations in computing resources. (2) The proposed method requires supplementary memory allocation for storing a few instances, rendering it susceptible to the constraints of storage capacity.

==> section/relation.tex <==
Speech is an important part of multimodality and the main medium of communication in daily life. Speech event detection is crucial for multimedia retrieval as it forms the basis for accurate indexing and access to large amounts of audiovisual content. In this paper, we study the speech event detection task in a continual learning scenario. We propose a cross-modality continual learning method, the input is speech and the output is text. This method is suitable for the encoder-decoder Transformer architecture. It can be easily applied to pre-trained models of text and visual modalities and helps to alleviate the catastrophic forgetting problem in continual multimodal learning tasks.

==> table/inbox.tex <==
\begin{table}[H]
    \caption{Dataset statistics.}
    \label{tab:dataset}
    \centering
    \resizebox{.48 \textwidth}{!}{
        \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
            \toprule
            \multirow{2}{*}{Task} & \multicolumn{3}{c|}{Speech ACE05} & \multicolumn{3}{c|}{Speech MAVEN} & \multicolumn{3}{c}{ESC-50} 
            \\ \cline{2-10} 
            & Event Type & Instance & Audio length & Event Type & Instance & Audio length & Event Type & Instance & Audio length \\ 
            \midrule
            1 & 2 & 1766 & 4.89 & 3 & 2999 & 11.22 & 10 & 400 & 0.56 \\ 
            2 & 2 & 1632 & 4.67 & 8 & 4561 & 17.07 & 10 & 400 & 0.56 \\ 
            3 & 6 & 1528 & 4.33 & 4 & 3476 & 13.01 & 10 & 400 & 0.56 \\ 
            4 & 4 & 1956 & 5.59 & 4 & 1909 & 7.14 & 10 & 400 & 0.56 \\ 
            5 & 3 & 1568 & 4.48 & 4 & 1542 & 5.77 & 10 & 400 & 0.56 \\ 
            6 & 3 & 1466 & 4.19 & 3 & 2346 & 8.78 & - & - & - \\ 
            7 & 2 & 1732 & 4.95 & - & - & - & - & - & - \\ 
            \bottomrule
        \end{tabular}
    }
\end{table}





\begin{table}[H]
    \caption{Hybrid data construction.}
    \label{tab:ch4-datasets-cg}
    \centering
    \resizebox{.48 \textwidth}{!}{
        \begin{tabular}{c|c|c|c|c|c|c}
            \toprule
            \multirow{2}{*}{Task} & \multicolumn{2}{c|}{Event Type} & \multicolumn{2}{c|}{Speech splicing} & \multicolumn{2}{c}{Speech overlay} \\ \cline{2-7} 
            & Semantic Event & Sound Event & Instance & Audio length & Instance & Audio length \\ 
            \midrule
            1 & conflict & nature & 2169 & 9.18 & 2169 & 6.16 \\ 
            2 & movement & nature & 1057 & 4.47 & 1057 & 3.01 \\ 
            3 & scenario & animal & 6955 & 29.42 & 6955 & 19.72 \\ 
            4 & talk & human & 4695 & 19.86 & 4695 & 13.34 \\ 
            \bottomrule
        \end{tabular}
    }
\end{table}

==> table/task-order-ace.tex <==
\begin{table}[H]
    \caption{Random different task sequences on Speech ACE05.}
    \label{tab:data-task-order-ace}
    \centering
    \resizebox{.68 \textwidth}{!}{
        \begin{tabular}{c|c}
            \toprule
            \textbf{Order} & \textbf{Task Sequence} \\ 
            \midrule
            1 & $ conflict \rightarrow contact \rightarrow justice \rightarrow movement \rightarrow personnel \rightarrow transaction \rightarrow life $  \\ 
            2 & $ personnel \rightarrow life \rightarrow contact \rightarrow conflict \rightarrow transaction \rightarrow justice \rightarrow movement $  \\ 
            3 & $ personnel \rightarrow conflict \rightarrow contact \rightarrow transaction \rightarrow justice \rightarrow life \rightarrow movement $  \\ 
            4 & $ movement \rightarrow justice \rightarrow transaction \rightarrow life \rightarrow conflict \rightarrow personnel \rightarrow contact $  \\ 
            5 & $ personnel \rightarrow life \rightarrow movement \rightarrow conflict \rightarrow contact \rightarrow transaction \rightarrow justice $  \\ 
            \bottomrule
        \end{tabular}
    }
\end{table}


\begin{table}[H]
    \caption{The mean of overall performance accuracy on Speech ACE05.}
    \label{tab:res-task-order-ace}
    \centering
    \resizebox{.58 \textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
        \toprule
        \textbf{Order} & \textbf{T1} & \textbf{T2} & \textbf{T3} & \textbf{T4} & \textbf{T5} & \textbf{T6} & \textbf{T7} & \textbf{Avg} \\ 
        \midrule
        \#1 & $82.00$ & $50.10$ & $38.67$ & $34.83$ & $26.26$ & $10.63$ & $26.13$ & $38.37$ \\ 
        \#2 & $52.00$ & $58.25$ & $46.97$ & $42.70$ & $26.08$ & $35.28$ & $36.29$ & $42.51$ \\ 
        \#3 & $52.00$ & $57.80$ & $43.00$ & $27.25$ & $34.49$ & $39.25$ & $36.83$ & $41.52$ \\ 
        \#4 & $89.00$ & $60.75$ & $39.60$ & $43.50$ & $35.80$ & $31.30$ & $34.73$ & $47.81$ \\ 
        \#5 & $52.00$ & $58.25$ & $53.07$ & $45.22$ & $36.64$ & $25.75$ & $34.01$ & $43.56$ \\ 
        \bottomrule
    \end{tabular}
    }
\end{table}



==> table/task-order-esc-v2.tex <==
\begin{table}[H]
    \caption{Random different task sequences on ESC-50.}
    \label{tab:data-task-order-esc}
    \centering
    \resizebox{.48 \textwidth}{!}{
        \begin{tabular}{c|c}
            \toprule
            \textbf{Order} & \textbf{Task Sequence} \\ 
            \midrule
            1 & $ animal \rightarrow domestic \rightarrow human \rightarrow nature \rightarrow urban $  \\ 
            2 & $ domestic \rightarrow nature \rightarrow human \rightarrow urban \rightarrow animal $  \\ 
            3 & $ domestic \rightarrow urban \rightarrow nature \rightarrow animal \rightarrow human $  \\ 
            4 & $ animal \rightarrow urban \rightarrow nature \rightarrow human \rightarrow domestic $  \\ 
            5 & $ domestic \rightarrow urban \rightarrow animal \rightarrow human \rightarrow nature $  \\ 
            \bottomrule
        \end{tabular}
    }
\end{table}

\begin{table}[H]
    \caption{The mean of overall performance accuracy on ESC-50.}
    \label{tab:res-task-order-esc}
    \centering
    \resizebox{.48 \textwidth}{!}{
        \begin{tabular}{c|c|c|c|c|c|c}
            \toprule
            \textbf{Order} & \textbf{T1} & \textbf{T2} & \textbf{T3} & \textbf{T4} & \textbf{T5} & \textbf{Avg ACC} \\
            \midrule
            \#1 & $81.00 $ & $76.85 $ & $67.87 $ & $69.38 $ & $66.52 $ & $72.32 $ \\
            \#2 & $85.00 $ & $70.00 $ & $72.10 $ & $69.40 $ & $68.82 $ & $73.06 $ \\
            \#3 & $85.00 $ & $71.25 $ & $62.00 $ & $69.47 $ & $67.50 $ & $71.04 $ \\
            \#4 & $81.00 $ & $72.60 $ & $68.27 $ & $64.12 $ & $59.02 $ & $69.00 $ \\
            \#5 & $85.00 $ & $71.25 $ & $62.90 $ & $64.93 $ & $64.94 $ & $69.80 $ \\
            \bottomrule
        \end{tabular}
    }
\end{table}


\begin{table}[H]
    \caption{Random different task sequences on Speech ACE05.}
    \label{tab:data-task-order-ace}
    \centering
    \resizebox{.58 \textwidth}{!}{
        \begin{tabular}{c|c}
            \toprule
            \textbf{Order} & \textbf{Task Sequence} \\ 
            \midrule
            1 & $ animal \rightarrow domestic \rightarrow human \rightarrow nature \rightarrow urban $  \\ 
            2 & $ domestic \rightarrow nature \rightarrow human \rightarrow urban \rightarrow animal $  \\ 
            3 & $ domestic \rightarrow urban \rightarrow nature \rightarrow animal \rightarrow human $  \\ 
            4 & $ animal \rightarrow urban \rightarrow nature \rightarrow human \rightarrow domestic $  \\ 
            5 & $ domestic \rightarrow urban \rightarrow animal \rightarrow human \rightarrow nature $  \\ 
            \bottomrule
        \end{tabular}
    }
\end{table}

\begin{table}[H]
    \caption{Random different task sequences on Speech MAVEN.}
    \label{tab:data-task-order-maven}
    \centering
    \resizebox{.58 \textwidth}{!}{
        \begin{tabular}{c|c}
            \toprule
            \textbf{Order} & \textbf{Task Sequence} \\ 
            \midrule
            1 & $ animal \rightarrow domestic \rightarrow human \rightarrow nature \rightarrow urban $  \\ 
            2 & $ domestic \rightarrow nature \rightarrow human \rightarrow urban \rightarrow animal $  \\ 
            3 & $ domestic \rightarrow urban \rightarrow nature \rightarrow animal \rightarrow human $  \\ 
            4 & $ animal \rightarrow urban \rightarrow nature \rightarrow human \rightarrow domestic $  \\ 
            5 & $ domestic \rightarrow urban \rightarrow animal \rightarrow human \rightarrow nature $  \\ 
            \bottomrule
        \end{tabular}
    }
\end{table}

==> table/task-order-maven.tex <==
\begin{figure}[!htbp]
\begin{minipage}[t]{0.48\textwidth}
    \centering
    \centering
    \resizebox{ \textwidth}{!}{
        \begin{tabular}{c|c}
            \toprule
            \textbf{Order} & \textbf{Task Sequence} \\ 
            \midrule
            1 & $ process \rightarrow action \rightarrow scenario \rightarrow move \rightarrow life \rightarrow talk $  \\ 
            2 & $ action \rightarrow process \rightarrow move \rightarrow life \rightarrow scenario \rightarrow talk $  \\ 
            3 & $ scenario \rightarrow process \rightarrow action \rightarrow move \rightarrow life \rightarrow talk $  \\ 
            4 & $ move \rightarrow talk \rightarrow action \rightarrow process \rightarrow life \rightarrow scenario $ \\ 
            \bottomrule
        \end{tabular}
    }
    \caption{Random different task sequences on Speech MAVEN.}
    \label{tab:data-task-order-maven}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
    \centering
    \resizebox{ \textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c}
        \toprule
        \textbf{Order} & \textbf{T1} & \textbf{T2} & \textbf{T3} & \textbf{T4} & \textbf{T5} & \textbf{T6} & \textbf{Avg ACC} \\ 
        \midrule
        \#1 & $86.00$ & $74.40$ & $64.00$ & $57.10$ & $52.46$ & $51.67$ & $64.27$ \\
        \#2 & $76.00$ & $72.35$ & $61.90$ & $56.50$ & $54.52$ & $53.23$ & $62.42$ \\
        \#3 & $82.00$ & $69.20$ & $65.10$ & $55.78$ & $53.18$ & $52.87$ & $63.02$ \\
        \#4 & $79.00$ & $70.35$ & $62.33$ & $61.65$ & $55.34$ & $50.97$ & $63.27$ \\
        \bottomrule
    \end{tabular}
    }
    \caption{The mean of overall accuracy on Speech MAVEN.}
    \label{tab:res-task-order-maven}
\end{minipage}
\end{figure}
